MIMIC: Masked Image Modeling with Image Correspondences

Dense pixel-specific representation learning at scale has been bottlenecked due to the unavailability of large-scale multi-view datasets. Current methods for building effective pretraining datasets heavily rely on annotated 3D meshes, point clouds, and camera parameters from simulated environments, preventing them from building datasets from real-world data sources where such metadata is lacking. We propose a pretraining dataset-curation approach that does not require any additional annotations. Our method allows us to generate multi-view datasets from both real-world videos and simulated environments at scale. Specifically, we experiment with two scales: MIMIC-1M with 1.3M and MIMIC-3M with 3.1M multi-view image pairs. We train multiple models with different masked image modeling objectives to showcase the following findings: Representations trained on our automatically generated MIMIC-3M outperform those learned from expensive crowdsourced datasets (ImageNet-1K) and those learned from synthetic environments (MULTIVIEW-HABITAT) on two dense geometric tasks: depth estimation on NYUv2 (1.7%), and surface normals estimation on Taskonomy (2.05%). For dense tasks which also require object understanding, we outperform MULTIVIEW-HABITAT, on semantic segmentation on ADE20K (3.89%), pose estimation on MSCOCO (9.4%), and reduce the gap with models pre-trained on the object-centric expensive ImageNet-1K. We outperform even when the representations are frozen, and when downstream training data is limited to few-shot. Larger dataset (MIMIC-3M) significantly improves performance, which is promising since our curation method can arbitrarily scale to produce even larger datasets. MIMIC code, dataset, and pretrained models are open-sourced at https://github.com/RAIVNLab/MIMIC.

==> old/00_abstract_v1.tex <==


\edit{\sout{Many pixel-wise dense prediction tasks—depth estimation and semantic segmentation—in computer vision today rely on pre-trained image representations.
Therefore, curating effective pretraining datasets is vital.}
Dense pixel-specific representation learning at scale has been bottlenecked due to the unavailability of large-scale multi-view datasets.}
The current methods to build effective pretraining datasets \edit{so far \sout{are those with multi-view scenes and}} heavily rely on annotated 3D meshes, point clouds, and camera parameters from simulated environments \edit{which prevents them from adapting to the real-world data sources where this metadata are lacking}. 
\edit{\sout{We propose a pretraining dataset-curation mechanism from videos of real scenes and synthetic 3D environments that does not require any annotations.}
We propose a pretraining dataset-curation mechanism that does not require any additional annotations. Our method seamlessly integrates with both--videos of real scenes and simulated environments.}
We mine two pretraining datasets: \datasetsmall with $1.3$M and \datasetlarge with $3.1$M  multi-view image pairs from open-sourced video datasets \edit{($32\%$)} and from synthetic 3D environments \edit{($68\%$)}.
We train multiple \edit{\sout{self-supervised}} models with different masked image modeling objectives to showcase the following findings:
\edit{Representations trained on \datasetlarge outperform those on real sources via crowdsourcing methods (ImageNet-1K) and synthetic sources mined using annotations (\baseline) on two geometric vision tasks -- depth estimation ( +6.19 $\delta1$ on NYUv2), and surface normals ( +1.11 L1 on Taskonomy). They also surpass the synthetic \baseline on object-related tasks such as semantic segmentation ( +1.58 mIOU on ADE20K), image classification (+$2.64\%$ on ImageNet-1K), and pose estimation (+6.3 AP and +5.2 AR on MSCOCO)} They outperform representations that are frozen and when downstream training data is limited to few-shot.
% Our ablations find that longer pretraining improves task performance.
Larger dataset (\datasetlarge) significantly improves performance, which is promising since our curation method can arbitrarily scale to produce even larger datasets.
